k2U: A General Framework from k-Point Effective Schedulability Analysis to Utilization-Based Tests

To deal with a large variety of workloads in different application domains in real-time embedded systems, a number of expressive task models have been developed. For each individual task model, researchers tend to develop different types of techniques for deriving schedulability tests with different computation complexity and performance. In this paper, we present a general schedulability analysis framework, namely the k2U framework, that can be potentially applied to analyze a large set of real-time task models under any fixed-priority scheduling algorithm, on both uniprocessor and multiprocessor scheduling. The key to k2U is a k-point effective schedulability test, which can be viewed as a "blackbox" interface. For any task model, if a corresponding k-point effective schedulability test can be constructed, then a sufficient utilization-based test can be automatically derived. We show the generality of k2U by applying it to different task models, which results in new and improved tests compared to the state-of-the-art. Analogously, a similar concept by testing only k points with a different formulation has been studied by us in another framework, called k2Q, which provides quadratic bounds or utilization bounds based on a different formulation of schedulability test. With the quadratic and hyperbolic forms, k2Q and k2U frameworks can be used to provide many quantitive features to be measured, like the total utilization bounds, speed-up factors, etc., not only for uniprocessor scheduling but also for multiprocessor scheduling. These frameworks can be viewed as a "blackbox" interface for schedulability tests and response-time analysis.

==> grm.tex <==
\section{Introduction}

For multiprocessor sporadic task systems, the capacity-augmentation factor for global RM is proved to be $2.668$ in this paper. We also provide tighter analysis than the existing result by Bertogna et al. \cite{DBLP:conf/opodis/BertognaCL05} by considering both the total utilization of the task system and the maximum task utilization in the schedulability test.



\subsection{Improved Analysis for Global RM}
\label{sec:global-sporadic}

To get better analysis than the solution in Theorem~\ref{thm:multiprocessor-GRM}, we need a better sufficient test than the naive sufficient test in Lemma~\ref{lemma:gRM-sufficient}. The following lemma provides a sufficient test based on the observations by Baruah et al. \cite{DBLP:journals/rts/BaruahBMS10}, in which the proof is in Appendix B.  


\begin{lemma}
\label{lemma:multiprocessor-grm-sporadic-pushforward} 
Let $U_k^{\max}$ be $\max_{j=1}^{k} U_j$. 
Task $\tau_k$ in a sporadic task system with implicit deadlines  is schedulable by global RM on
$M$ processors if
\begin{align*}
  \forall y \geq 0, \forall 0 \leq \omega_i \leq T_i, \exists t \mbox{ with } 0 < t \leq T_k+y  {\;\; and \;\;} \\
  U_k^{\max} \cdot(T_k+y) +
 \frac{ \sum_{i=1}^{k-1} \omega_i\cdot U_i+ \ceiling{\frac{t-\omega_i }{T_i}} C_i
}{M}\leq t.
\end{align*}
\end{lemma}

The schedulability condition in Lemma~\ref{lemma:multiprocessor-grm-sporadic-pushforward} requires to test all possible $y \geq 0$ and all possible settings of $0 \leq \omega_i \leq T_i$ for the higher priority tasks $\tau_i$ with $i=1,2,\ldots,k-1$. At first glance, it may seem to be difficult to use the \framework{} framework. It requires some further annotation before adopting the framework, as shown in the proof of the following theorem.

\begin{theorem}
  \label{thm:multiprocessor-grm-sporadic-tight}
Let $U_k^{\max}$ be $\max_{j=1}^{k} U_j$.  
Task $\tau_k$ in a sporadic task system with implicit deadlines  is schedulable by global RM on
$M$ processors if
\begin{equation}
\label{eq:schedulability-GRM-tight}
(U_k^{\max} +1) \prod_{j=1}^{k-1} (\frac{U_j}{M} + 1)\leq 2,
\end{equation}
or
\begin{equation}
\label{eq:schedulability-GRM-tight-ubound}
\sum_{j=1}^{k-1} \frac{U_j}{M}\leq \ln{\frac{2}{U_k^{\max}  +1}}.
\end{equation}
\end{theorem}
\begin{proof}
  We will show that the schedulability condition in the theorem holds for all possible settings of $y$ and $\omega_i$s.
  Suppose that $y$ and $\omega_i$ for $i=1,2,\ldots,k-1$  are given, in which  $y \geq 0$ and $0 \leq \omega_i \leq T_i$. Let $t_k$ be $T_k+y$. Now, we set $t_i$ to $\omega_i + \floor{\frac{T_k+y-\omega_i}{T_i}}T_i$ for $i=1,2,\ldots,k-1$ and reindex the tasks such that $t_1 \leq t_2 \leq \ldots \leq t_k$. The sufficient schedulability condition in Lemma~\ref{lemma:multiprocessor-grm-sporadic-pushforward} under the given $y$ and $\omega_i$s is to verify the existence of $t_j \in
\setof{t_1, t_2, \ldots t_k}$ such that
\begin{align}
  &U_k^{\max}(T_k+y) + \frac{\sum_{i=1}^{k-1}  \omega_i\cdot U_i+ \ceiling{\frac{t_j-\omega_i }{T_i}} C_i}{M} \\ 
 \leq & U_k^{\max} t_k + \frac{\sum_{i=1}^{k-1} U_i t_i + \sum_{i=1}^{j-1} C_i}{M} 
  \leq t_j.  
\end{align}
\jj{bug from here!!!}
  By the definition of $t_i$ and  $y \geq 0$ and the global RM scheduling (i.e., $T_k \geq T_i$), we can conclude that $t_i \geq T_k+y \geq T_i$, which implies that $C_i \leq U_i t_i$.
  Hence, we know that the sufficient test is to verify whether there exists
 $t_j \in
\setof{t_1, t_2, \ldots t_k}$ such that
\begin{align}
  \label{eq:final-grm-k2u-precondition}
U_k^{\max} t_k + \sum_{i=1}^{k-1} \alpha_i U_i t_i + \sum_{i=1}^{j-1} \beta_i U_i t_i
  \leq t_j,
\end{align}
where $\alpha_i = \frac{1}{M}$ and $\beta_i \leq \frac{1}{M}$ for $i=1,2,\ldots,k-1$.
Therefore, we reach the conclusion of the schedulability conditions in Eqs.~\eqref{eq:schedulability-GRM-tight} and \eqref{eq:schedulability-GRM-tight-ubound} by Lemma~\ref{lemma:framework-constrained} and
Lemma~\ref{lemma:framework-totalU-exclusive} under given $y$ and $\omega_i$s.\footnote{The concern that $y$ may be unbounded (so may $t_k$) can be handled by normalizing all the $t_i$ values for higher priority tasks $\tau_i$s to $t_k$ and set $t_k$ to $1$ after the normalization. }

The schedulability test in Eq.~\eqref{eq:final-grm-k2u-precondition} is independent from the settings of $y$ and $\omega_i$s. However, the setting of $y$ and $\omega_i$s affects how the $k-1$ higher priority tasks are indexed. Fortunately, it can be observed that the schedulability tests in Eqs.~\eqref{eq:schedulability-GRM-tight} and \eqref{eq:schedulability-GRM-tight-ubound} are completely independent upon the indexing of the higher priority tasks. Therefore, no matter how $y$ and $\omega_i$s are set, the schedulability conditions in Eqs.~\eqref{eq:schedulability-GRM-tight} and \eqref{eq:schedulability-GRM-tight-ubound} are the corresponding results from the \framework{} framework.
As a result, we can reach the conclusion.
\end{proof}

\begin{corollary}
  \label{col:grm-tight}
  The capacity augmentation factor of global RM for a sporadic system with implicit deadlines is $2.668$.
\end{corollary}
\begin{proof}
  Suppose that $\sum_{\tau_i} \frac{C_i}{M T_i} \leq \frac{1}{b}$ and
  $U_k \leq \max_{\tau_i} U_i \leq
  \frac{1}{b}$.  Therefore, by
  Eq.~\eqref{eq:schedulability-GRM-tight-ubound}, we can guarantee
  the schedulability of task $\tau_k$ if $\frac{1}{b} \leq
  \ln{\frac{2}{1+\frac{1}{b}}}$. This is equivalent to solving $x =
  \ln{\frac{2}{1+x}}$, which holds when $x\approx
  2.668$ by solving the equation numerically. Therefore,
  we reach the conclusion of the capacity augmentation factor
  $2.668$.
\end{proof}

{\bf Remarks:} The utilization bound in Eq.~\eqref{eq:schedulability-GRM-tight-ubound} is analytically better than the best known utilization-based schedulability test $\sum_{j=1}^{k} U_j\leq \frac{M}{2}(1-U_k^{\max})+U_k^{\max}$ for global RM by Bertogna et al. \cite{DBLP:conf/opodis/BertognaCL05}, since $\frac{(1-x)}{2} \leq \ln\frac{2}{1+x}$ when $0 \leq x \leq 1$. The capacity augmentation factor $2.668$ in Corollary \ref{col:grm-tight} is the same as the result by Lundberg \cite{DBLP:conf/rtas/Lundberg02}. As shown in \cite{DBLP:conf/rtas/Lundberg02}, the factor $2.668$ is tight when the number of tasks is sufficiently large.

We would like to point out the incompleteness in the proof in \cite{DBLP:conf/rtas/Lundberg02}. In the proof of the extreme task set, the argument in Page 150 in \cite{DBLP:conf/rtas/Lundberg02} concludes that task $\tau_n$ is more difficult to be schedulable due to the increased interference of task $\tau_{n-1}$ to task $\tau_n$ after the transformation. The argument was not correctly proved since the increased interference has to be analyzed in all time points in the analysis window, whereas the analysis in \cite{DBLP:conf/rtas/Lundberg02} only considers the interference in a specific interval length. Without analyzing the resulting interference in all time points in the analysis window, task $\tau_n$ after transformation may still have chance to finish earlier due to the potential reduction of the interference at earlier time points.

We limit our attention here for the global RM scheduling. Andersson et al. \cite{DBLP:conf/rtss/AnderssonBJ01} propose the RM-US[$\varsigma$] algorithm, which gives the highest priority to tasks $\tau_i$s with $U_i > \varsigma$, and otherwise assigns priorities by using RM. Our analysis here can also be applied for the RM-US[$\varsigma$] algorithm with some modifications in the proofs by setting $\varsigma=\frac{1}{2.668}\approx 0.37482$.



\begin{appProof}{Lemma~\ref{lemma:multiprocessor-grm-sporadic-pushforward}}
  This is proved by contrapositive. If task $\tau_k$ is not schedulable by global RM, we will show that there exist $y \geq 0$ and $0 \leq \omega_i \leq T_i$ such that for all $0 < t \leq T_k+y$, the condition $U_k^{\max} \cdot (T_k+y) +
 \frac{ \sum_{i=1}^{k-1} \omega_i\cdot U_i+ \ceiling{\frac{t-\omega_i }{T_i}} C_i
}{M} > t$ holds. The proof is mainly based on the forwarding algorithm for the analysis of global DM by Baruah et al. in \cite{DBLP:journals/rts/BaruahBMS10}, by making some further annotations.

  If $\tau_k$ is not schedulable, let $z_0$ be the first time that task $\tau_k$ misses its absolute deadline, i.e., $z_0$.  Let $z_1$ be the arrival time of this job of task $\tau_k$.  For notational brevity, let this job be $J_1$, which arrives at time $z_1$ and has not yet been finished at time $z_0$. By definition, we know that $z_0-z_1$ is $T_k$. Due to the scheduling policy and the implicit-deadline setting, removing (1) all the other jobs of task $\tau_k$ (except the one arriving at time $z_1$), (2) all the jobs arriving no earlier than $z_0$,  and (3) lower-priority jobs does not change the unschedulability of job $J_1$. Therefore, all the jobs that are considered for the rest of the proof come from $\tau_1, \tau_2, \ldots, \tau_k$.

  Now, we expand the interval of interest by using a slightly different algorithm from that proposed in \cite{DBLP:journals/rts/BaruahBMS10}, also illustrated with the notations in Figure~\ref{fig:force-forward}, as follows:
 \begin{algorithm}[h]
   \label{alg:feasibility-analysis2}
    \begin{algorithmic}[1]\small
        \FOR {$\ell\leftarrow2,3,...$}
          \STATE let $J_\ell$ denote a job that 
          \begin{compactitem}[-]
          \item arrives at some time-instant $z_\ell<z_{\ell-1}$;
          \item has an absolute deadline after $z_{\ell-1}$;
          \item has not completed execution by $z_{\ell-1}$; and
          \item has executed for strictly less than $(z_{\ell-1}-z_\ell)\cdot \hat{U}_\ell$
	 units over the interval $[z_\ell,z_{\ell-1})$, where $\hat{U}_\ell$ is the utilization of the task that generates job $J_\ell$.
          \end{compactitem}

          \IF {there is no such a job}
          \STATE $\ell\leftarrow (\ell-1)$; break;
          \ENDIF
      \ENDFOR
     \end{algorithmic}
     \end{algorithm}

     Suppose that the forwarding algorithm terminates with $\ell$ equals to $\ell^*$. We now examine the schedule in the interval $(z_{\ell^*}, z_0]$. Since $J_1, J_2, \ldots, J_{\ell^*}$ belong to $\tau_1, \tau_2, \ldots, \tau_k$, we know that $\hat{U}_\ell \leq U_k^{\max}$ for $\ell=1,2,\ldots,\ell^*$. Let $\sigma_\ell$ be the total length of the time interval over $(z_\ell, z_{\ell-1}]$ during which $J_\ell$ is executed. By the choice of $J_\ell$, it follows that
     \[
     \sigma_\ell < (z_{\ell-1}-z_{\ell}) \cdot \hat{U}_\ell.
     \]
     Moreover, all the $M$ processors execute other higher-priority jobs (than $J_\ell$) at any other time points in the interval $(z_\ell, z_{\ell-1}]$ at which $J_\ell$ is not executed.
     Therefore, by the above analysis, we know that the maximum amount of time from $z_{\ell^*}$ to $z_0$, in which not all the $M$ processors execute certain jobs, is at most
     \begin{align*}
       \sum_{\ell=1}^{\ell^*} \sigma_\ell &<      \sum_{\ell=1}^{\ell^*} (z_{\ell-1}-z_{\ell}) \cdot \hat{U}_\ell\\
       &\leq
     \sum_{\ell=1}^{\ell^*} (z_{\ell-1}-z_{\ell}) \cdot U_k^{\max} = (z_0-z_{\ell^*}) \cdot U_k^{\max}.       
   \end{align*}

   Now, we replace job $J_0$ with job $J_0'$ in the above schedule, where $J_0'$ is released at time $z_{\ell^*}$ with absolute deadline $z_0$ and execution time $(z_0-z_{\ell^*}) \cdot U_k^{\max}$. According to the above analysis, $J_0'$ cannot be finished before $z_{0}$ in the above schedule.
   For each task $\tau_i$ for $i=1,2,\ldots,k-1$, in the above schedule, there may be one \emph{carry-in} job, denoted as $J_i^\flat$, of $\tau_i$ that arrives at time $r_i^\flat$ with $r_i^\flat < z_{\ell^*}$ and has absolute deadline after $d_i^\flat$ with $d_i^\flat > z_{\ell^*}$. According to the termination condition in the construction of $z_{\ell^*}$, if $J_i^\flat$ exists, we know that at least $(z_{\ell^*}-r_i^\flat)\cdot U_i$ amount of execution time has been executed before $z_{\ell^*}$, and the remaining execution time of job $J_i^\flat$ to be executed after $z_{\ell^*}$ is at most
   $(d_i^\flat - z_{\ell^*})\cdot U_i$. If $J_i^\flat$ does not exist, then $d_i^\flat$ is set to $z_{\ell^*}$ for notational brevity. Therefore, the amount of workload $W_i'(t)$ of all the released jobs of task $\tau_i$ for $i=1,2,\ldots,k-1$ to be executed in time interval $(z_\ell^*, z_\ell^*+t)$ is at most
   \begin{equation}
     \label{eq:1}
   W_i'(t)  = (d_i^\flat - z_{\ell^*})\cdot U_i+ \ceiling{\frac{t-(d_i^\flat - z_{\ell^*}) }{T_i}} C_i.     
   \end{equation}
   Clearly, this is more precise than the naive time demand function $W_i(t)$ in Eq.~\eqref{eq:W_i-multiprocessor}.
   
   The assumption of the unschedulability of job $J_0'$ (due to the unschedulability of job $J_0$) under global RM implies that $J_0'$ cannot finish its computation at any time between $z_{\ell^*}$ and $z_0$. This leads to the following (necessary) condition 
  $U_k^{\max} (z_0-z_{\ell^*}) +
  \frac{ \sum_{\tau_i \in hp(\tau_k)}W_i'(t) }{M} >  t$ for all $0 < t \leq z_{\ell^*}-z_0$ for the unschedulability of job $J_0'$.   Therefore, by the existence of $y=z_{0}-z_{\ell^*}$ and $\omega_i = d_i^\flat - z_{\ell^*}$ for $i=1,2,\ldots, k-1$ to force the above necessary condition, we reach the conclusion of the proof by contrapositive. 
\end{appProof}

\begin{figure}[t]
  \centering
  \scalebox{0.45}{
    \begin{tikzpicture}[x=1cm,font=\sffamily\Large,ultra thick]]
   
  \draw[->](0,0) -- (19, 0)  node[right]{$x$};
  
   \draw[-](2,-.1) node[below]{$z_\ell$} -- (2, 1)  -- (5,1) node[pos=.5,above]{$J_\ell$} -- (5,0) ;
     
    \draw[-](4,-.1) node[below]{$z_{\ell-1}$} -- (4, 1.2)  -- (7,1.2) node[pos=.5,above]{$J_{\ell-1}$};

\draw[-](10,1) node[above]{$J_{3}$} -- (13,1) -- (13,0) ;

 \draw[-](12,-.1) node[below]{$z_2$} -- (12, 1.2)  -- (16,1.2) node[pos=.5,above]{$J_2$} -- (16,0) ;

 \draw[-](15,-.1) node[below]{$z_1$} -- (15, 1)  -- (18,1) node[pos=.5,above]{$J_1$} -- (18,0)node[below]{$z_0$} ;
 
  \node [ ] at (8,0.6) {$\cdot\cdot\cdot\cdot\cdot$};
    \node [ ] at (1,0.6) {$\cdot\cdot\cdot\cdot\cdot$};
      \end{tikzpicture}  }
  \caption{Notations of the forwarding algorithm for the analysis of global RM.}
  \label{fig:force-forward}
\end{figure}


==> kevin.tex <==
%%Cut to here by JJ on 26,08,2014

\subsection{Response Time Bound in Fixed-Priority Scheduling with Arbitrary Deadlines}
\begin{definition}[Last Release]
For a given task $\tau_i$ in the interval
$[\phi,\phi+D_n)$ for any $\phi \ge 0$, $t_i$ denotes the time of the last release of task $\tau_i$.

\begin{lemma}
  \label{lemma:response-time-unschedulability}
Let $X^*$ denote the time at which the $k^{th} job$ of $\tau_n$ misses its deadline.
If the $k^{th}$ job of task $\tau_n$ misses its deadline, then
    \begin{equation*}   
\forall \tau_i,\quad kC_n+\sum_{i=1}^{n-1}U_it_i+\sum_{j=1}^{i-1}C_j> t_i
    \end{equation*}
 \end{lemma}
\begin{proof}

\end{proof}
\end{definition}
\begin{definition}[Worst-Case Response Time]
$R_n=X^*-(k-1)T_n$
\end{definition}
\begin{theorem}
The worst-case reponse time $R_n$ of task $\tau_n$ is bounded above by 
\begin{align*}
 R_n\le \frac{C_n+\sum_{i=1}^{n-1}C_i-\sum_{i=1}^{n-1}(U_i\sum_{j=i}^{n-1}C_j)}{1-\sum_{i=1}^{n-1}U_i}
\end{align*}
where tasks are indexed with 
\begin{equation*}
\forall \tau_i \quad \frac{C_{i+1}}{U_{i+1}}<\frac{C_{i}}{U_{i}}.
\end{equation*}
\end{theorem}
\begin{proof}
We prove this theorem by finding the supremum $R_n$ subject to the conditions in
 Lemma~\ref{lemma:response-time-unschedulability}.
This is a strictly convex problem. Since we have more variables than constraints, 
all of the constraints have to be \emph{active} according to the extreme point theorem.
\begin{equation*}
kC_n+\sum_{i=1}^{n-1}U_i(t_1+\sum_{j=1}^{i-1}C_j)= t_1
\end{equation*}
\begin{align*}
t_1&=\frac{kC_n+\sum_{i=1}^{n-1}(U_i\sum_{j=1}^{i-1}C_j)}{1-\sum_{i=1}^{n-1}U_i}\\
&\ge 0 \quad \text{($\sum_{i=1}^nU_i<1$)}
\end{align*}
Then, the response time is bounded by
\begin{equation}
\label{eq:response-time-supermum-k}
R_n\le \frac{kC_n+\sum_{i=1}^{n-1}C_i-\sum_{i=1}^{n-1}(U_i\sum_{j=i}^{n-1}C_j)}{1-\sum_{i=1}^{n-1}U_i}-(k-1)T_n.
\end{equation}
We now prove the maximum in Eq. (\ref{eq:response-time-supermum-k}) occur for $k=1$. 
\begin{align*}
\frac{d}{dk}&\left(\frac{kC_n+\sum_{i=1}^{n-1}C_i-\sum_{i=1}^{n-1}(U_i\sum_{j=i}^{n-1}C_j)}{1-\sum_{i=1}^{n-1}U_i}-(k-1)T_n\right)\\
&=\frac{C_i}{1-\sum_{i=1}^{n-1}U_i}-T_n\\
&=T_n(\frac{U_i}{1-\sum_{i=1}^{n-1}U_i}-1)\\
&=T_n(\frac{\sum_{i=1}^{n}U_i-1}{1-\sum_{i=1}^{n-1}U_i})
\end{align*}
which is negative since our assumption $\sum_{i=1}^{n}U_i<1$. Since this function is decreasing, the maximum occurs in the left bound, which means $k=1$. 
By substituting $k=1$ in Eq. (\ref{eq:response-time-supermum-k}), this theorem follows.
\end{proof}
\subsection{Response Time Bound in Fixed-Priority Scheduling with Arbitrary Deadlines with unknown $C$}
\begin{lemma}
Let $X^*$ denote the time at which the $k^{th} job$ of $\tau_n$ misses its deadline.
If the $k^{th}$ job of task $\tau_n$ misses its deadline, then
    \begin{equation*}   
\forall \tau_i,\quad kC_n+\sum_{i=1}^{n-1}U_it_i+\sum_{j=1}^{i-1}U_jt_j> t_i
    \end{equation*}
 \end{lemma}
\begin{theorem}
If 
\begin{equation*}
\prod_{i=1}^{n} (U_i + 1)\le2,
\end{equation*}
then the worst-case reponse time $R_n$ of task $\tau_n$ is bounded above by 
\begin{equation*}
R_n\le \frac{C_n}{\frac{2}{\prod_{i=1}^{n-1} (U_i + 1)}-1}.
\end{equation*}
\end{theorem}
\begin{proof}
\begin{equation}
t_{i}U_i= t_{i+1}-t_i.
\end{equation}

\begin{align*}
&kC_n+\sum_{i=1}^{n-1}U_it_i= t_1\\
\Rightarrow &kC_n+t_n-t_1= t_1\\
\Rightarrow &kC_n+t_1\prod_{i=1}^{n-1} (U_i + 1)-t_1= t_1\\
\Rightarrow &t_1=\frac{kC_n}{2-\prod_{i=1}^{n-1} (U_i + 1)}
\end{align*}
\begin{align*}
R_n&\le kC_n+2\sum_{i=1}^{n-1}U_it_i-(k-1)T_n\\
&= kC_n+2(t_1\prod_{i=1}^{n-1} (U_i + 1)-t_1)-(k-1)T_n\\
&=kC_n+\frac{2kC_n(\prod_{i=1}^{n-1} (U_i + 1)-1)}{2-\prod_{i=1}^{n-1} (U_i + 1)}-(k-1)T_n\\
&=\frac{kC_n\prod_{i=1}^{n-1} (U_i + 1)}{2-\prod_{i=1}^{n-1} (U_i + 1)}-(k-1)T_n\\
&=\frac{kC_n}{\frac{2}{\prod_{i=1}^{n-1} (U_i + 1)}-1}-(k-1)T_n\\
\end{align*}
We now prove the maximum in Eq. (\ref{eq:response-time-supermum-k}) occur for $k=1$. 
\begin{align*}
\frac{d}{dk}&\left(\frac{kC_n}{\frac{2}{\prod_{i=1}^{n-1} (U_i + 1)}-1}-(k-1)T_n\right)\\
&=\frac{C_n}{\frac{2}{\prod_{i=1}^{n-1} (U_i + 1)}-1}-T_n\\
&=T_n(\frac{U_n}{\frac{2}{\prod_{i=1}^{n-1} (U_i + 1)}-1}-1)\\
&=T_n(\frac{U_n\prod_{i=1}^{n-1} (U_i + 1)}{2-\prod_{i=1}^{n-1} (U_i + 1)}-1)\\
&=T_n(\frac{U_n\prod_{i=1}^{n-1} (U_i + 1)-2+\prod_{i=1}^{n-1} (U_i + 1)}{2-\prod_{i=1}^{n-1} (U_i + 1)})\\
&=T_n(\frac{\prod_{i=1}^{n} (U_i + 1)-2}{2-\prod_{i=1}^{n-1} (U_i + 1)})\\
\end{align*}
\end{proof}
